MolRecBench-Wild: A Real-World Benchmark for Optical Chemical Structure Recognition

Optical Chemical Structure Recognition (OCSR) aims to translate molecular diagrams in scientific literature into machine-readable formats, but current systems remain unreliable on real-world images due to substantial visual and chemical complexity. We introduce MOSAIC, a dual-dimensional difficulty framework with 37 fine-grained labels that jointly characterize visual interference and chemical semantic challenges in molecular diagrams. Based on this framework, we construct MolRecBench-Wild, a benchmark of 5,029 structures from 820 recent chemistry papers, covering the full difficulty spectrum observed in real publications. To enable faithful semantic evaluation beyond SMILES and MolFile, we propose CARBON, a representation language capable of expressing valence variations, icon-based groups, and other non-standard chemical semantics. We further adopt a dual-track evaluation protocol supporting both CARBON and SMILES outputs for broad model compatibility. Comprehensive experiments over 18 OCSR-capable models reveal severe performance degradation on MolRecBench-Wild, exposing a large gap between previous patent benchmarks and real-world academic scenarios.

==> table/visual_dimension.tex <==
\begin{table}[]
\begin{tabular}{lllllllll}
Hardcase   id        & Hardcase Name                                           & Images               & Hardcase id          & Hardcase Name                                                        & Images               & Hardcase id          & Hardcase Name                                                              & Images               \\
                     & {\color[HTML]{D83931} }                                 &                      &                      & {\color[HTML]{D83931} }                                              &                      &                      & {\color[HTML]{D83931} }                                                    &                      \\
\multirow{-2}{*}{1}  & \multirow{-2}{*}{{\color[HTML]{D83931} Decorated Text}} & \multirow{-2}{*}{\#} & \multirow{-2}{*}{2}  & \multirow{-2}{*}{{\color[HTML]{D83931} Decorated Bond}}              & \multirow{-2}{*}{\#} & \multirow{-2}{*}{3}  & \multirow{-2}{*}{{\color[HTML]{D83931} Polluted Boundary}}                 & \multirow{-2}{*}{\#} \\
                     & {\color[HTML]{D83931} }                                 &                      &                      & {\color[HTML]{D83931} }                                              &                      &                      & {\color[HTML]{D83931} }                                                    &                      \\
\multirow{-2}{*}{4}  & \multirow{-2}{*}{{\color[HTML]{D83931} Blurry Image}}   & \multirow{-2}{*}{\#} & \multirow{-2}{*}{5}  & \multirow{-2}{*}{{\color[HTML]{D83931} Additional Arrow, Box, Text}} & \multirow{-2}{*}{\#} & \multirow{-2}{*}{6}  & \multirow{-2}{*}{{\color[HTML]{D83931} Colored Areas or Image Background}} & \multirow{-2}{*}{\#} \\
                     & {\color[HTML]{D83931} }                                 &                      &                      & {\color[HTML]{D83931} }                                              &                      &                      & {\color[HTML]{D83931} }                                                    &                      \\
\multirow{-2}{*}{7}  & \multirow{-2}{*}{{\color[HTML]{D83931} Bond Crossing}}  & \multirow{-2}{*}{\#} & \multirow{-2}{*}{8}  & \multirow{-2}{*}{{\color[HTML]{D83931} R Represented by Pattern}}    & \multirow{-2}{*}{\#} & \multirow{-2}{*}{9}  & \multirow{-2}{*}{{\color[HTML]{D83931} Colored Ar}}                        & \multirow{-2}{*}{\#} \\
                     & {\color[HTML]{D83931} }                                 &                      &                      & {\color[HTML]{D83931} }                                              &                      &                      & {\color[HTML]{D83931} }                                                    &                      \\
\multirow{-2}{*}{10} & \multirow{-2}{*}{{\color[HTML]{D83931} Short Bond}}     & \multirow{-2}{*}{\#} & \multirow{-2}{*}{11} & \multirow{-2}{*}{{\color[HTML]{D83931} Numbered Atom}}               & \multirow{-2}{*}{\#} & \multirow{-2}{*}{12} & \multirow{-2}{*}{{\color[HTML]{D83931} Incomplete Molecule}}               & \multirow{-2}{*}{\#} \\
                     & {\color[HTML]{D83931} }                                 &                      &                      & {\color[HTML]{D83931} }                                              &                      &                      & {\color[HTML]{D83931} }                                                    &                      \\
\multirow{-2}{*}{13} & \multirow{-2}{*}{{\color[HTML]{D83931} Large Molecule}} & \multirow{-2}{*}{\#} & \multirow{-2}{*}{14} & \multirow{-2}{*}{{\color[HTML]{D83931} Large Font}}                  & \multirow{-2}{*}{\#} & \multirow{-2}{*}{15} & \multirow{-2}{*}{{\color[HTML]{D83931} Long Bond}}                         & \multirow{-2}{*}{\#} \\
                     & {\color[HTML]{D83931} }                                 &                      &                      & {\color[HTML]{D83931} }                                              &                      &                      & {\color[HTML]{D83931} }                                                    &                      \\
\multirow{-2}{*}{16} & \multirow{-2}{*}{{\color[HTML]{D83931} Thick Bond}}     & \multirow{-2}{*}{\#} & \multirow{-2}{*}{17} & \multirow{-2}{*}{{\color[HTML]{D83931} Thin Bond}}                   & \multirow{-2}{*}{\#} & \multirow{-2}{*}{18} & \multirow{-2}{*}{{\color[HTML]{D83931} Long Functional Group Name}}        & \multirow{-2}{*}{\#}
\end{tabular}
\end{table}
